Neural Machine Translation for Bilingually Scarce Scenarios: A Deep Multi-task Learning Approach

Neural machine translation requires large amounts of parallel training text to learn a reasonable-quality translation model. This is particularly inconvenient for language pairs for which enough parallel text is not available. In this paper, we use monolingual linguistic resources in the source side to address this challenging problem based on a multi-task learning approach. More specifically, we scaffold the machine translation task on auxiliary tasks including semantic parsing, syntactic parsing, and named-entity recognition. This effectively injects semantic and/or syntactic knowledge into the translation model, which would otherwise require a large amount of training bitext. We empirically evaluate and show the effectiveness of our multi-task learning approach on three translation tasks: English-to-French, English-to-Farsi, and English-to-Vietnamese.

==> sec50-aux-tasks.tex <==
%The motivation behind the proposed architecture is to effectively inject directly semantic and/or syntactic knowledge into the translation. The model provides a framework to share knowledge among tasks in each component (encoder/decoder). Also, by partly sharing components, each task also would be able to learn its own task-specific skills in each component. We chose the following auxiliary tasks to provide the model with the related knowledge for enhancing the quality of translation.

\begin{itemize}[leftmargin=5mm]

\item \textbf{Named-Entity Recognition (NER)}: With the low amount of bilingual pairs it would be hard for the model to learn how to translate rarely occurring named-entities. By learning NER task, the model learn the skill to recognize the named-entities, it would then be more feasible for it to find out the underlying pattern for translating them e.g for some named-entities it should just transliterate (mostly for person names and dates) or translate words (mostly organization names). \textbf{Named-Entity Recognition}: TBD(Conll NER task dataset)

\item \textbf{Semantic Parsing}: A good translation should preserve the meaning. By learning semantic parsing task the model learns the skill to abstract the meaning of the source sentence, which also would be beneficial in the translation task. For this task, the model learn to parse English sentences into Abstract Meaning Representation (AMR) graphs.  \textbf{Semantic Parsing}: TBD (AMR corpus v2)

\item \textbf{Syntactic constituency parsing}: This task is added to learn the model the ability to identify the phrase structure of the input sentence. When the model is able to recognize phrases and their types, it would be easier for it to learn the relocation in the target language.  \textbf{Syntactic Parsing}: TBD (PennTree bank (standard))
\end{itemize}

%if we try to learn a multitask model with related tasks to translation, the auxiliary tasks will serve as helpful sources for inductive bias. Also, we can see it as learning sub-skills in the auxiliary task which would be useful for the main task (or other tasks). 

%One approach for MTL for improving MT (can we claim this as ours?) is to share the whole components (encoder and/or decoder). When encoder is shared, it may learn a general skill to capture the information related to all tasks from the source sentence. When the decoder is shared, it may learn to recognize the task in hand and use the required skills. Using MTL with this architecture has better performance than single-task learning. However, we propose a new architecture which is carefully designed for MTL in Seq2Seq neural transduction models to enable components learn shared and task-specific sub-skills separately. In the proposed architecture, the bottom layers of components (encoder and/or decoder) are shared while top layers are task-specific. This architecture provides each component with the ability to learn both general and task-specific sub-skills efficiently. This architecture biases each component towards learning a general-purpose internal representations on the bottom layers which is able to capture all of the required information for all tasks. It can be explained as learning general sub-skills in the lower layers and task-specific sub-skills in the higher ones. For example, if we learn translation along with named-entity recognition as auxiliary task. The model may learn a general purpose sub-skill to recognize dates in the lower levels, while the translation-related skills in the higher levels will recognize and add information about the event corresponding to the date in the internal representation of it on the top layers.




